MotionGRPO: Overcoming Low Intra-Group Diversity in GRPO-Based Egocentric Motion Recovery

This paper studies full-body 3D human motion recovery from head-mounted device signals. Existing diffusion-based methods often rely on global distribution matching, leading to local joint reconstruction errors. We propose MotionGRPO, a novel framework leveraging reinforcement learning post-training to inject fine-grained guidance into the diffusion process. Technically, we model diffusion sampling as a Markov decision process optimized via Group Relative Policy Optimization (GRPO). To this end, we introduce a hybrid reward mechanism that combines a learned conditioned perceptual model for global visual plausibility and explicit constraints for local joint precision. Our key technical insight is that policy optimization in diffusion-based recovery suffers from vanishing gradients due to limited intra-group sample diversity. To address this, we further introduce a noise-injection strategy that explicitly increases sample variance and stabilizes learning. Extensive experiments demonstrate that MotionGRPO achieves state-of-the-art performance with superior visual fidelity

==> equations/mtd_1.tex <==
\begin{align}
    \text{d}\mathbf{x} = \mathbf{f}(x, t) \text{d}t + g(t)\text{d}\mathbf{w}
\end{align}

==> equations/mtd_2.tex <==
\begin{align}
    \text{d}\mathbf{x}_t = (\mathbf{f}(\mathbf{x}, t)- \frac{1+\epsilon_t^{2}}{2}g(t)^2\nabla \log \ p_t(\mathbf{x}_t))\text{d}t + \epsilon_t \text{d} \mathbf{w}
\end{align}


==> equations/mtd_3.tex <==
\begin{align}
&\mathcal{J}_{GRPO} = \nonumber \\ 
&\mathbb{E} \left[ \frac{1}{G} \sum_{i=1}^G \frac{1}{N} \sum_{t=1}^T  \left( \frac{\pi_\theta(o_{i,t}|\mathbf{c})}{\pi_{old}(o_{i,t}|\mathbf{c})} \hat{A}_{i,t} - \omega_{\text{KL}} \mathbb{D}_{\text{KL}} \right) \right] 
\label{eq:grpo}
\end{align}


==> equations/mtd_rwd_1.tex <==
\begin{align}
    \text{d}\mathbf{x} = \mathbf{f}(x, t) \text{d}t + g(t)\text{d}\mathbf{w}
\end{align}

==> fig/vis-Head.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{fig/icml-vis-0127.pdf}
    \vspace{-0.3cm}
    \caption{\textbf{Qualitative Comparison and Visualization} The first row presents a qualitative comparison with the most competitive baseline on the AMASS dataset. Red boxes highlight failure cases, such as ground penetration and inaccurate joint positions. The second row visualizes the results of \projecttitle\ on the ADT dataset, demonstrating its generalization capability to real-world scenarios.}
    \label{fig: vis}
    \vspace{-0.5cm}
\end{figure*}

==> sec/0_abstract.tex <==
\begin{abstract}
Here is abstract
\end{abstract}
